UNBOX: Unveiling Black-box visual models with Natural-language

Ensuring trustworthiness in open-world visual recognition requires models that are interpretable, fair, and robust to distribution shifts. Yet modern vision systems are increasingly deployed as proprietary black-box APIs, exposing only output probabilities and hiding architecture, parameters, gradients, and training data. This opacity prevents meaningful auditing, bias detection, and failure analysis. Existing explanation methods assume white- or gray-box access or knowledge of the training distribution, making them unusable in these real-world settings. We introduce UNBOX, a framework for class-wise model dissection under fully data-free, gradient-free, and backpropagation-free constraints. UNBOX leverages Large Language Models and text-to-image diffusion models to recast activation maximization as a purely semantic search driven by output probabilities. The method produces human-interpretable text descriptors that maximally activate each class, revealing the concepts a model has implicitly learned, the training distribution it reflects, and potential sources of bias. We evaluate UNBOX on ImageNet-1K, Waterbirds, and CelebA through semantic fidelity tests, visual-feature correlation analyses and slice-discovery auditing. Despite operating under the strictest black-box constraints, UNBOX performs competitively with state-of-the-art white-box interpretability methods. This demonstrates that meaningful insight into a model's internal reasoning can be recovered without any internal access, enabling more trustworthy and accountable visual recognition systems.

==> UNBOX/tables/ablation.tex <==
A key question in understanding the behaviour of \methodname{} is how much of its performance depends on the auxiliary components introduced in Sec. \ref{sec:method}.
While the semantic optimisation mechanism can operate using only trend-based signals, the full method also incorporates two additional elements:
(i) the Global Optimization Context ($P_{best}$, $D_{best}$), which aggregates long-term semantic evidence; and
(ii) the intensity state $I_t$, which modulates the strength of textual refinements.
The ablation study in Table \ref{tab:ablation_study} evaluates the contribution of these components and clarifies whether they are necessary for stable and semantically meaningful convergence.

The evaluation, ran on a subset of 10 classes, uses the same three criteria adopted in the main results:
\begin{enumerate}
    \item descriptor–label similarity ($DL$), assessing Semantic Class Fidelity (Sec. \ref{sec:fidelity});
	\item	descriptor–data similarity ($DD$), assessing alignment with data-derived descriptors as defined in  (Sec. \ref{sec:latent});
	\item	descriptor–image similarity ($DI$), assessing visual grounding on validation images (Sec. \ref{sec:latent}).
\end{enumerate}

When both the Global Optimization Context and the intensity state are disabled, performance is consistently low across all three measures (0.50, 0.30, 0.42).
This shows that trend-based optimisation alone is insufficient and leads to unstable or incoherent descriptors.

Enabling only the intensity state yields partial gains, particularly in descriptor–data similarity (from 0.30 to 0.60).
This indicates that controlling the magnitude of semantic refinements helps reduce oscillations, but does not fully anchor the optimisation to the model’s learned concepts.

When both components are active, performance improves substantially across all metrics (0.90 on descriptor–label and descriptor–data similarity, 0.87 on descriptor–image similarity).
This demonstrates that the Global Optimization Context provides essential long-range semantic structure: it accumulates stable cues, prevents semantic drift, and reinforces refinements that consistently increase the class activation.
Combined with intensity-aware adjustment, these mechanisms enable \methodname{} to consistently recover descriptors that are semantically faithful, grounded in the training distribution, and visually aligned with the classifier’s behaviour under strict black-box constraints.


\begin{table}[h!]
    \centering
    %\small 
    
    \rowcolors{2}{table-gray}{white}
     \renewcommand{\arraystretch}{1.2}
    \setlength{\tabcolsep}{10.5pt}  
    \caption{Ablation study evaluating the contributions of the Global Optimization Context $(P_{best}, D_{best})$ and the intensity state $I_t$ to the overall performance.}
    \label{tab:ablation_study}
       
    \begin{tabular}{ccccc}
        \toprule
        \rowcolor{white} 
        \boldmath$P_{best}, D_{best}$ & \boldmath$I_t$ & \textbf{DL} & \textbf{DD} & \textbf{DI} \\
        \midrule
        
        \xmark & \xmark & 0.50 & 0.30 &  0.42\\ 
        \xmark & \checkmark & 0.50 & 0.60 & 0.40 \\
        \checkmark & \checkmark & 0.90 & 0.90 & 0.87 \\
        \bottomrule
    \end{tabular}
\end{table}


==> UNBOX/tables/descriptors_zero_shot.tex <==
\begin{table}[t]
    \centering
    %\small 
    

    \rowcolors{1}{table-gray}{white}
    
\caption{Alignment between generated descriptors and data-derived semantic attributes.  
Scores quantify the similarity between each method’s descriptors and keywords extracted from captioned training images, reflecting how well the recovered semantics match the distribution the classifier was trained on. Columns W and D denote access to model weights and data, respectively.  Higher values indicate stronger data-grounded semantic recovery. As DEXTER and \methodname{} are non-deterministic, results are averaged over three runs.}    \label{tab:data_der_zero_shot}
    
    \renewcommand{\arraystretch}{1.4}
    
    \begin{tabular}{l c c c c }
        \toprule
        \rowcolor{white} 
        \textbf{Method} & \textbf{W} & \textbf{D}  & \textbf{RN50} & \textbf{ViT} \\
        \midrule
        
        WWW \cite{ahn2024unified}            & \checkmark & \checkmark          & 0.43          & 0.27 \\
        CLIPDissect \cite{oikarinen2023clipdissect}    & \checkmark & \checkmark & 0.73  & 0.30 \\
        DEXTER \cite{carnemolla2025dexter}         & \checkmark & \xmark       & $0.49\pm0.01$  
        & $0.34\pm0.01$     \\
        \methodname     & \xmark     & \xmark             & $0.63\pm0.04$         &  $0.45\pm0.03$   \\
        Random          & \xmark     & \xmark              & 0.03        & 0.03 \\
        
        \bottomrule
    \end{tabular}
\end{table}





==> UNBOX/tables/human_evaluation.tex <==
\begin{table}[h]
    \centering
    \caption{Results of the user study}
    \label{tab:results}
    \begin{tabular}{lcc}
        \toprule
        \textbf{Method} & \textbf{Q1} & \textbf{Q2} \\
        \midrule
        WWW \cite{ahn2024unified}      & 3.29$\pm$1.33 & 3.20$\pm$1.43 \\
        CLIPDissect \cite{oikarinen2023clipdissect}  & \textbf{4.05}$\pm$0.96 & \textbf{3.96}$\pm$1.10 \\
        DEXTER \cite{carnemolla2025dexter} & 3.67$\pm$1.22 & 3.04$\pm$1.51 \\
        \methodname & \ul{3.73}$\pm$1.15 & \ul{3.68}$\pm$1.30 \\
        \bottomrule
    \end{tabular}
\end{table}

==> UNBOX/tables/image_zero_shot.tex <==


\begin{table}[htbp]
    \centering
    
    
    
    \rowcolors{1}{table-gray}{white}
    
\caption{Visual grounding evaluation on ImageNet-1K.  
Generated descriptors are used as textual queries over validation images to assess how strongly they correspond to concrete visual evidence.  Columns W and D denote access to model weights and data, respectively.
Ground-truth labels (GT) serve as an upper bound. As DEXTER and \methodname{} are non-deterministic, results are averaged over three runs. \label{tab:image_zero_shot}}
    
    \renewcommand{\arraystretch}{1.4}
    
    \begin{tabular}{l c c c c  }
        \toprule
        \rowcolor{white} 
        \textbf{Method} & \textbf{W} & \textbf{D} & \textbf{RN50} & \textbf{ViT} \\
        \midrule
        
        GT (Labels)     & -        & -         & 0.90 & 0.90 \\
        GT (Descr.)& \xmark     & \checkmark              & 0.76       & 0.76          \\
        WWW \cite{ahn2024unified}            & \checkmark     & \checkmark         & 0.66       & 0.63          \\
        CLIPDissect \cite{oikarinen2023clipdissect}     & \checkmark     & \checkmark     & 0.85 & 0.36          \\
        DEXTER \cite{carnemolla2025dexter}          & \checkmark     & \xmark         & $0.42\pm0.01$             & $0.36\pm0.02$              \\
        \methodname     & \xmark     & \xmark       & $0.56\pm0.04$ & $0.43\pm0.04$             \\
        Random          & \xmark     & \xmark               & 0.03                 & 0.03          \\
        
        \bottomrule
    \end{tabular}
\end{table}

==> UNBOX/tables/labels_zero_shot.tex <==
\begin{table}[htbp]
    \centering

    \rowcolors{1}{table-gray}{white}   
    \caption{Class semantic fidelity evaluation: similarity between generated descriptors and ImageNet-1K class labels on three architectures. Columns W and D denote access to model weights and data, respectively.  Higher values indicate stronger alignment with the ground-truth class concept. As DEXTER and \methodname{} are non-deterministic, results are averaged over three runs.}
    \label{tab:labels_zero_shot}

    \renewcommand{\arraystretch}{1.4}
    \begin{tabular}{l c c c c}
        \toprule
        \rowcolor{white} 
        \textbf{Method} & \textbf{W} & \textbf{D} & \textbf{RN50} & \textbf{ViT} \\
        \midrule
        WWW \cite{ahn2024unified}          & \checkmark & \checkmark         & 0.60        & 0.40 \\
        CLIPDissect \cite{oikarinen2023clipdissect}     & \checkmark & \checkmark      & 0.77 & 0.27 \\
        DEXTER \cite{carnemolla2025dexter}         & \checkmark & \xmark             & $0.47\pm0.03$             & $0.34\pm0.01$            \\
        \methodname     & \xmark     & \xmark      & $0.64\pm0.09$ & $0.49\pm0.04$    \\
        Random          & \xmark     & \xmark             & 0.03       & 0.03 \\
        \bottomrule
    \end{tabular}
\end{table}  

==> UNBOX/tables/slice_discovery.tex <==
\begin{table*}[htbp]
    \centering
    \small 
    \setlength{\tabcolsep}{4pt} 
    
    
    \rowcolors{3}{table-gray}{white}
    
    \caption{Comparison of slice discovery and debiasing performance on the Waterbirds and CelebA benchmarks. 
    Metrics include worst-group (\textit{Worst}) and average (\textit{Avg}) accuracy.\label{tab:slice_discovery}}
    
    \renewcommand{\arraystretch}{1.3}
    
    \begin{tabular}{lccccccc}
        \toprule
        \rowcolor{white}
        & & & & \multicolumn{2}{c}{\textbf{Waterbirds}} & \multicolumn{2}{c}{\textbf{CelebA}} \\
        \cmidrule(lr){5-6} \cmidrule(lr){7-8}
        
        \rowcolor{white}
        \textbf{Method} & \textbf{Weights} & \textbf{Data} & \textbf{GT} & \textbf{Worst} & \textbf{Avg} & \textbf{Worst} & \textbf{Avg} \\
        \midrule
        
        ERM       & \checkmark & \checkmark & \xmark      & 62.6$\pm$0.3 & 97.3 & 47.7$\pm$2.1 & 94.9 \\
        LfF \cite{nam2020learning}     & \checkmark & \checkmark & \xmark      & 78.0         & 91.2 & 77.2         & 85.1 \\
        GEORGE \cite{sohoni2020no}  & \checkmark & \checkmark & \xmark      & 76.2$\pm$2.0 & 95.7 & 54.9$\pm$1.9 & 94.6 \\
        JTT \cite{liu2021just}     & \checkmark & \checkmark & \xmark      & 83.8$\pm$1.2 & 89.3 & 81.5$\pm$1.7 & 88.1 \\
        CNC \cite{zhang2022correct}    & \checkmark & \checkmark & \xmark      & 88.5$\pm$0.3 & 90.9 & 88.8$\pm$0.9 & 89.9 \\
        DRO  \cite{sagawadistributionally}    & \checkmark & \checkmark & \checkmark & 89.9$\pm$1.3 & 91.5 & 90.0$\pm$1.5 & 93.3 \\
        LADDER \cite{ghosh2025ladder}  & \xmark      & \checkmark & \xmark      & 92.4$\pm$0.8 & 93.1 & 89.2$\pm$0.4 & 89.8 \\
        DRO B2T \cite{kim2024discovering}  & \xmark      & \checkmark & \xmark     & 90.7$\pm$0.3 & 92.1 & 90.4$\pm$0.9 & 93.2 \\
        DEXTER \cite{carnemolla2025dexter}  & \checkmark & \xmark      & \xmark      & 90.5$\pm$0.1 & 92.0 & 91.3$\pm$0.01 & 91.7 \\
        \methodname & \xmark   & \xmark      & \xmark      & 	88.6$\pm$0.2        & 91.0&    90.01$\pm$0.3         &  90.91   \\
        
        \bottomrule
    \end{tabular}
\end{table*}

==> UNBOX/tex/ablation.tex <==
\label{ablation}
\input{tables/ablation}

==> UNBOX/tex/conclusion.tex <==
\label{conclusion}

We introduced \methodname{}, a framework for class-wise model dissection that operates under the strictest black-box constraints: access is limited solely to output probabilities, with no gradients, features, model weights, or training data. By reformulating activation maximization as a semantic optimization problem in text space, \methodname{} combines a trend- and intensity–driven guidance mechanism with an LLM-based refinement process that iteratively constructs natural-language descriptors for a target class. A global and local optimization context further stabilizes the search, enabling the recovery of coherent and persistent semantic cues.

Extensive experiments demonstrate that \methodname{} achieves high semantic class fidelity, reliably identifying the concepts associated with a target class from output probabilities alone. The method also recovers latent training semantics, uncovering features genuinely grounded in the data distribution and reflected in the classifier’s visual decision patterns. Despite its strict black-box setting, \methodname{} matches or surpasses state-of-the-art white-box and grey-box dissection tools across multiple architectures, including CNNs and Vision Transformers.

Beyond semantic recovery, \methodname{} provides a principled mechanism for bias discovery. By extracting fine-grained contextual descriptors and using them to construct slice-aware pseudo-labels, the method supports effective debiasing through standard robust optimization techniques. On Waterbirds and CelebA, the discovered descriptors yield worst-group accuracies competitive with or approaching methods that require full access to model internals or training data, and in some cases rival the performance of oracle group labels.

Taken together, these findings show that meaningful model dissection and auditing are possible even when models are accessible only through an inference API. \methodname{} offers a general semantic lens for inspecting the behaviour, implicit training signals, and systematic biases of modern visual classifiers, opening the door to new forms of transparent, data-free, and architecture-agnostic model analysis.


==> UNBOX/tex/experiments/dataset_metrics.tex <==
Our experiments are designed to answer three questions: 
(1) how accurately \methodname{} can recover the concept associated with a target class using only output probabilities (Semantic Fidelity); 
(2) whether the recovered descriptors reflect the latent semantics encoded in the model's training distribution (Latent Training Semantics Recovery); and 
(3) whether the method can reveal spurious correlations and coherent dataset slices (Bias Discovery). 
All evaluations use established vision benchmarks and compare \methodname{} against the most recent state-of-the-art methods under standardized protocols.\\

\noindent \textbf{Datasets.} For Semantic Fidelity and Latent Training Semantics Recovery, we use the ImageNet-1K validation set, restricted to the 30-class subset introduced by \cite{carnemolla2025dexter}, following the 15 spurious / 15 non-spurious split defined by Salient ImageNet \cite{singla2021salient}.

For Bias Discovery, we use the standard CelebA \cite{liu2015deeplearningfaceattributes} and Waterbirds \cite{sagawadistributionally} benchmarks, as done in recent slice-discovery and debiasing work \cite{yu2025error, kim2024discovering, ghosh2025ladder, nam2020learning, sohoni2020no, liu2021just, zhang2022correct, carnemolla2025dexter}. CelebA contains over 200k face images annotated with 40 binary attributes, while Waterbirds introduces background-related spurious correlations by compositing bird images onto mismatched environments.\\

\noindent \textbf{Models investigated.} We evaluate \methodname{} on two representative and structurally divergent classifiers:
(1) \emph{ResNet50}, a convolutional architecture with strong locality and hierarchical feature extraction, and 
(2) \emph{ViT-B/16}, a transformer-based model that relies on global self-attention with markedly different inductive biases.
These two models were selected not as a limitation of the approach, but to demonstrate that a purely output-driven semantic optimization procedure can generalize across fundamentally different visual processing mechanisms.
Since \methodname{} operates on the output probabilities of a classifier, it can be applied to \emph{any} image classification model, regardless of architecture, modality of internal computation, or access to weights, while maintaining the same level of generality.\\

\noindent \textbf{Competitors.} We compare against CLIPDissect \cite{oikarinen2023clipdissect} and WWW \cite{ahn2024unified}, both of which provide neuron-level explanations but rely on weights and data access, and DEXTER \cite{carnemolla2025dexter}, a grey-box method requiring weights access. This positions \methodname{}---which operates solely from class probabilities---in a strictly more constrained setting. To ensure a fair comparison, we utilize the set of five class lexical units generated by \methodname{} (Sec. \ref{optimization_setup}). For the neuron-centric baselines (CLIPDissect and WWW), we construct an equivalent set by aggregating the top-4 penultimate-layer neuron lexical units and appending the descriptor from the classification head. We strictly adhere to their implementation guidelines, adopting the exact concept vocabularies: WordNet-20K for CLIPDissect and the 80,000 most frequent English words for WWW.  As the probing dataset for both, we employ the same validation set used for the visual grounding evaluation (Tab. \ref{tab:image_zero_shot}).
Unlike competing deterministic methods, DEXTER and \methodname{} are non-deterministic; therefore, we run the optimization three times and report the mean and standard deviation.
For bias and slice-discovery experiments, we compare against the current state-of-the-art methods used in robustness literature, including text-based methods such as B2T \cite{kim2024discovering} and LADDER \cite{ghosh2025ladder}, and with the standard DRO baseline \cite{sagawadistributionally}.\\

\noindent \textbf{Metrics.} Evaluation uses complementary semantic and visual metrics. 
Semantic Fidelity is measured by embedding-based similarity between generated descriptors and ground-truth labels using Sentence Transformers and CLIP. 
Latent Training Semantics Recovery is evaluated through descriptor-to-caption similarity and descriptor-to-image alignment, quantifying how well the recovered semantics reflect the model’s implicit training distribution. 
Bias Discovery is assessed using the standard slice-level accuracy, worst-group accuracy, and spurious-correlation detection metrics used in prior work.

==> UNBOX/tex/experiments/datasets.tex <==
\label{datasets}
All evaluations reported in Tab. \ref{tab:labels_zero_shot}, Tab. \ref{tab:data_der_zero_shot}, Tab. \ref{tab:image_zero_shot}, Tab. \ref{tab:results}, are carried out on the ImageNet-1K validation set, with respect to the 30-class subset used in \cite{carnemolla2025dexter}, chosen by following the 15 spurious/15 not spurious classification introduced by Salient ImageNet \cite{singla2021salient}. ImageNet \cite{deng2009imagenet} is a large-scale benchmark comprising millions of labeled natural images spanning a wide variety of object categories and a standard test-bed for evaluating visual models. 
We also make use of Salient ImageNet’s saliency-based analyses for selecting relevant neurons for the penultimate layer of models accessed by competitors CLIPDissect \cite{oikarinen2023clipdissect} and WWW \cite{ahn2024unified} when comparing our performance to theirs.

For slice discovery and debiasing (\ref{slice_discovery}), we adopt the CelebA \cite{liu2015deeplearningfaceattributes} and Waterbirds \cite{sagawadistributionally} datasets as benchmarks, as done in \cite{yu2025error, kim2024discovering, ghosh2025ladder, sagawadistributionally, nam2020learning, sohoni2020no, liu2021just, zhang2022correct, carnemolla2025dexter}, with results presented in Tab. \ref{tab:slice_discovery}. CelebA \cite {liu2015deeplearningfaceattributes} includes more than 200k face images annotated with 40 binary attributes capturing various identity-related and stylistic characteristics, such as \textit{gender}, \textit{age} and \textit{hair length}. For experiments, we follow the standard split of the dataset.
Waterbirds is a dataset introduced by the authors of DRO \cite{sagawadistributionally}, designed to study spurious correlations by compositing bird pictures, drawn from the Caltech-UCSD Birds-200-2011 (CUB) dataset, onto mismatched backgrounds (land vs. water).


==> UNBOX/tex/experiments/experiments_intro.tex <==
\label{experiments_intro}

==> UNBOX/tex/experiments/human_evaluation.tex <==
\label{human_evaluation}


==> UNBOX/tex/experiments/optimization_setup.tex <==
\label{optimization_setup}
For each class-wise dissection, we allocate a maximum of 1000 optimization steps, 
with early stopping triggered once the visual classifier predicts the target class 
for 10 consecutive generated images. Images are produced using 
\texttt{black-forest-labs/FLUX.1-schnell}~\cite{flux2024} with a single diffusion step, 
while all agents ($A_f$ and $A_u$) operate on \texttt{gpt-oss:120b}~\cite{openai2025gptoss120bgptoss20bmodel}. 
On a system equipped with two H100 GPUs---one handling image synthesis and classifier 
queries, the other dedicated to LLM inference---each optimization step requires 
approximately 15 seconds.

The trend--state tolerance is set to $\varepsilon = 10^{-4}$, and the thresholds 
controlling intensity-state discretization ($\tau_{\text{high}}$) and global-context 
accumulation ($\tau_{\text{best}}$) are set to $10^{-2}$ for standard class-optimization 
experiments. For slice-discovery tasks, which require less sensitivity to small 
probability variations, both thresholds are set to $9 \times 10^{-1}$. The global context 
retains the top $m = 5$ lexical units extracted from high-scoring prompts, while 
the local optimization context stores the previous $k = 10$ prompt--feedback pairs.

Prompt initialization follows the task setting: standard class dissection begins 
from the generic template ``\texttt{a picture of a random object}'', whereas slice 
discovery uses a domain-aware initialization, 
``\texttt{a picture of a [DOMAIN]}'' (e.g., ``\texttt{a picture of a bird}'' for 
Waterbirds).  




==> UNBOX/tex/experiments/semantic_class_fidelity.tex <==

A fundamental question in model dissection is whether the recovered descriptors truly identify the intended concept associated with a target class. For a black-box setting such as ours, where no gradients, features, or training data
are available, this becomes particularly challenging: the method must infer a class-level semantic description using only the scalar probability returned by the model. An evaluation of \emph{semantic class fidelity} therefore serves as the
most direct test of whether \methodname{} has successfully uncovered the core semantics that the classifier associates with each class.

To assess this property, we compare the descriptors generated by
\methodname{} with the ground-truth ImageNet class labels. An effective dissection method should produce descriptors whose meaning is significantly closer to the correct class label than to unrelated alternatives. Concretely, we concatenate the top--5 descriptors produced for each class into a single
prompt, encode both descriptor and label using T5-XL, and compute their class semantic similarity.

\input{tables/labels_zero_shot}

We evaluate against three baselines representative of the current state of the
art. WWW and CLIPDissect are white-box methods that require full access to
model weights and a probing dataset; DEXTER is a grey-box method relying on
activation maximization over model weights alone. A random-word baseline is
reported as a lower-bound control.

Results in Tab.~\ref{tab:labels_zero_shot} show that \methodname{} achieves high semantic fidelity across all architectures despite operating under the
strictest constraints. 
On ResNet50, \methodname{} reaches an accuracy of 0.64 exceeding WWW while remaining competitive with CLIPDissect, that, however, requires access to data and models' weights. The advantage becomes even more evident on ViT models: \methodname{} achieves the highest score (0.49), dramatically outperforming CLIPDissect and WWW.

These results indicate that methods relying on internal activations or neuron probes may struggle to generalize across different architectural paradigms, while \methodname{}—driven purely by output probabilities—maintains stable and robust interpretability performance. This demonstrates that semantic
optimization in text space is not only feasible for black-box models but can match or surpass white-box competitors in recovering the core concept encoded by a class.



==> UNBOX/tex/experiments/semantic_recovery.tex <==
\input{tables/descriptors_zero_shot}
\input{tables/image_zero_shot}

While semantic fidelity assesses whether \methodname{} can identify the correct class from output probabilities alone, a core objective of model dissection is to determine whether the explanations capture the \emph{semantics the classifier actually learned from its training distribution}. A descriptor may sound plausible or natural-language–coherent without corresponding to attributes genuinely used by the model.
To address this, we evaluate whether the descriptors recovered by \methodname{} reflect (i) concepts present in the training data and (ii) visual patterns that meaningfully influence the classifier’s predictions.

\paragraph{Alignment with data-derived descriptors.}
A single class label is often insufficient to reveal the richness of the underlying data distribution: classes exhibit characteristic co-occurring features, contextual patterns and, in some cases, spurious cues.
To evaluate whether \methodname{} captures this broader semantic structure, we construct a set of data-derived descriptors by captioning 100 training images per class with LLaVA and extracting the most frequent informative keywords (after removing stop-words and non-semantic tokens).
These keywords form a data-grounded description of what appears in the training samples.

For each class, we concatenate the top-5 descriptors produced by \methodname{} and by the data-derived process into two respective prompts, encode them using T5-XL embeddings, and measure cosine similarity.
We compare against DEXTER, CLIPDissect, WWW, and a random-word baseline.

As shown in Tab.~\ref{tab:data_der_zero_shot}, CLIPDissect performs strongly due to its direct access to model weights and data. However, \methodname{} consistently ranks among the top performers despite operating under strict black-box constraints.
On ResNet50 it outperforms WWW; and on ViT—where internal activation probing used by white-box methods becomes less reliable: \methodname{} achieves the highest score overall.
These results indicate that \methodname{} uncovers features that reflect the distribution the classifier was trained on, rather than generating plausible but ungrounded explanations.

\paragraph{Visual grounding on validation images.}
Textual similarity alone cannot guarantee that recovered descriptors correspond to \emph{visually grounded} evidence in the data.
Therefore, we treat each descriptor as a pseudo-label and measure how well it aligns with ImageNet validation images of the corresponding class. This evaluates whether the descriptors encode features that are not only present in the training data but also consistently expressed in the model’s visual decision cues.

An important distinction is that CLIPDissect and WWW both rely on the validation set as probing data for concept extraction, whereas \methodname{} does not access any images during descriptor generation.
Thus, this experiment constitutes a stricter test for our method.

As shown in Tab.~\ref{tab:image_zero_shot}, \methodname{} demonstrates strong grounding performance.
On ResNet50, it nearly closes the gap with WWW; and on ViT, it substantially outperforms CLIPDissect, whose neuron-level probes degrade on transformer architectures.

These findings jointly indicate that \methodname{} recovers descriptors that are both semantically aligned with the model’s training distribution and visually grounded in the data. Despite having no access to model weights, gradients, or training images, the method uncovers latent semantic structure that white-box methods typically access only through internal activations.



==> UNBOX/tex/experiments/slice_disc.tex <==
The final component of our evaluation concerns whether \methodname{} can uncover
\emph{systematic spurious correlations} and identify dataset slices where the classifier fails.
Unlike class-level concept discovery, which targets stable defining features of a class,
slice discovery requires isolating subtle, fine-grained cues—such as backgrounds or demographic attributes—that influence predictions only within specific subsets of samples.

To focus the optimization on relevant variations, we initialize the search with a lightweight
domain prior (e.g., ``a picture of a bird'' for Waterbirds or ``a picture of a celebrity'' for CelebA).
This assumption reflects realistic auditing scenarios where the model’s exact taxonomy may be unknown,
but its application domain is typically evident.

\input{tables/slice_discovery}

Because spurious cues may be averaged out during global optimization,
we additionally extract instance-level descriptors.
Whenever a generated image $x_t$ activates the target class with high confidence,
we pass $x_t$ through a vision–language model (LLaVA) to obtain $k=5$
fine-grained visual descriptors.
Aggregating all descriptors collected throughout the optimization and ranking them by frequency
reveals the dominant slice-defining attributes for each class.
For Waterbirds, for example, this process naturally identifies ``branch'' for landbirds
and ``water'' for waterbirds, corresponding to the well-known background bias.

To validate that these descriptors accurately capture the spurious correlations affecting the classifier,
we incorporate them into a debiasing pipeline following B2T~\cite{kim2024discovering}.
Each descriptor is embedded using CLIP to build textual prototypes, which serve as
pseudo-labelers of the training data.
Images whose visual features align more strongly with the prototype of the opposite class
are annotated as belonging to the conflict slice.
These groups are then used to retrain a classifier with DRO~\cite{sagawadistributionally},
and the resulting worst-group accuracy provides a quantitative measure of the quality of our slice descriptors.

Table~\ref{tab:slice_discovery} reports worst-group accuracy on Waterbirds and CelebA.
On \emph{Waterbirds}, \methodname{} achieves 88.6 worst-group accuracy,
performing competitively with
white-box and data-dependent slice discovery methods, despite using only output probabilities.
On \emph{CelebA}, \methodname{} attains 90.01 worst-group accuracy, matching Oracle DRO and closely approaching DEXTER.

These results show that \methodname{} not only recovers class-defining concepts
and latent training semantics but also exposes the subtle, systematic biases that drive distribution shifts.
Despite operating under strict black-box constraints,
the discovered textual descriptors are sufficiently precise to enable effective debiasing on standard robustness benchmarks.

==> UNBOX/tex/experiments/slice_discovery_and_debiasing.tex <==
\label{slice_discovery}
The goal of \textbf{slice discovery} is to identify coherent subpopulations (slices) within a dataset where a model systematically underperforms compared to its average accuracy. This task is critical for auditing deep learning models, as these performance degradations are often symptomatic of reliance on \textit{spurious correlations}---non-causal features (e.g., background textures, lighting conditions, or demographic attributes) that happen to co-occur with the target label in the training distribution but fail to generalize.

\noindent\textbf{Task Specificity: From Concepts to Nuances.} This task differs fundamentally from the standard class optimization described in previous sections. In our standard setting, the goal is to recover \textit{generic} class features. In contrast, slice discovery requires identifying subtle, fine-grained nuances or contextual backgrounds (e.g., a "landbird" appearing on "water") that act as spurious attractors. These nuances are often sample-specific and less semantically dominant than the core class concept, making them harder to isolate with a purely aggregative prompt. To bridge this gap and achieve the necessary level of granularity, we introduce a specialized two-stage mechanism to our pipeline.

\noindent\textbf{Domain-Aware Initialization.} While our framework operates in a strict black-box setting, effective auditing requires a minimal semantic anchor. For the slice discovery task specifically, we assume knowledge of the \textbf{macro-domain} on which the classifier operates (e.g., ``birds'' for the Waterbirds dataset, or ``celebrities'' for CelebA).
We motivate this relaxation of the zero-knowledge constraint by considering the realistic workflow of an AI auditor: when auditing a proprietary API, the specific class taxonomy or training data may be unknown, but the \textit{function} of the model is known (e.g., an API sold as a "Face Verification Tool" inherently implies the domain of faces).
Leveraging this, we initialize the optimization not with a random prompt, but with a domain-specific template $p_0$ (e.g., ``\textit{a picture of a bird}'' for Waterbirds or ``\textit{a picture of a celebrity}'' for CelebA). This focuses the search space on relevant variations within the domain rather than exploring the entire semantic universe.

\noindent\textbf{Fine-Grained Descriptor Extraction via VLM.} To capture sample-specific nuances that might be averaged out in the global optimization prompt, we integrate an additional extraction step. Whenever a generated image $x_t$ successfully activates the target class during the optimization loop (i.e., is classified as the target with high confidence), it is passed to a Vision-Language Model (LLaVA).
We query LLaVA to extract $k=5$ specific visual descriptors from $x_t$. This allows us to record highly detailed, instance-level features (e.g., "forest," "water background") that triggered the classifier.

\noindent\textbf{Slice Identification via Ranking.} At the end of the process, rather than relying on the final optimized prompt, we aggregate all sample-specific descriptors collected from the successful images. These descriptors are ranked by frequency. The descriptor with the highest occurrence count for a given class is selected as the representative definition of the biased slice (e.g., identifying "branch" as the dominant spurious feature for Class 0 in Waterbirds, or "woman" for Class 1 in CelebA).

\noindent\textbf{Debiasing.} To quantitatively assess the quality and utility of our discovered slice descriptors, we employ a debiasing task. It is important to clarify that our primary goal here is not to propose a new debiasing algorithm per se, but rather to demonstrate that the descriptors extracted by \methodname{} accurately capture the spurious correlations affecting the model. If our descriptors effectively define the biased slices, they should enable the training of a robust classifier using standard mitigation techniques. 
Following the protocol established by B2T \cite{kim2024discovering}, we use the discovered text descriptors to generate pseudo-labels for the training data. Specifically, we construct zero-shot classifiers using CLIP. For each class, we create a textual prototype based on the dominant descriptor identified in the Slice Discovery phase. We then classify the training images against these prototypes. This step allows us to detect samples where the visual content aligns with the spurious feature of a conflicting class.

Let's consider the Waterbirds dataset as an illustrative example. This dataset contains two classes: Class 0 (``Landbird'') and Class 1 (``Waterbird''). Our slice discovery process identifies ``branch'' as the dominant descriptor for Class 0 and ``water'' for Class 1. We use these words to create CLIP embeddings.
During the annotation phase, if an image with the ground-truth label 0 (Landbird) is classified by CLIP as being closer to the prototype of the opposite class (``water''), it is annotated as ``sliced'' (belonging to a conflict group). This annotation signifies that the image contains the spurious background typically associated with the opposing class.

These generated pseudo-labels categorize the dataset into distinct groups based on the presence or absence of the spurious feature. We then utilize these groups to retrain a robust classifier using Distributionally Robust Optimization (DRO) \cite{sagawadistributionally}, which minimizes the worst-group loss. The performance of this retrained model serves as a proxy for the quality of our descriptors: high accuracy on the worst-group test set indicates that \methodname{} successfully identified the semantic attributes driving the distribution shift.

\subsubsection{Debiasing results}
The results of debiasing on the Waterbirds and CelebA benchmarks are summarized in Tab. \ref{tab:slice_discovery}. The performance of \methodname{} is compared against a suite of several state-of-the-art methods, ranging from standard training (ERM) to specialized slice discovery methods that rely on extensive access to model internals (DEXTER), training data (e.g., LADDER, B2T) or both (LfF, GEORGE, JTT, CNC). We also include Oracle DRO, which uses ground-truth group labels, serving as an upper bound for performance.

On the \textbf{Waterbirds} dataset, \methodname{} achieves a worst-group accuracy of 88.6. This represents a substantial improvement over the ERM baseline, demonstrating that our descriptors successfully identify the ``landbird on water'' and ``waterbird on land'' spurious correlations. Remarkably, our approach remains highly competitive with white-box and data-dependent methods. We perform comparably to the Oracle DRO, and are within striking distance of DEXTER and B2T, which requires full access to model weights. While LADDER achieves the highest performance, it crucially relies on access to the training data to mine slices, a requirement that \methodname{} circumvents entirely.

The results on \textbf{CelebA} further validate our approach. Here, \methodname{} achieves a worst-group accuracy of 90.01. This result is particularly significant as it effectively matches the performance of the Oracle DRO, proving that our discovered text descriptors are as effective for debiasing as the ground-truth annotations themselves. Furthermore, we remain very close to the state-of-the-art grey-box method DEXTER.

Overall, these experiments confirm that \methodname{} can uncover and define systematic model biases with high fidelity. Despite operating without access to weights, gradients, or training data, our framework generates descriptors that enable robust debiasing, bridging the gap between black-box auditing and white-box mitigation.


==> UNBOX/tex/experiments/spurious_discovery.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\textwidth]{figs/spurious_discovery.png}
    \caption{Qualitative examples of spurious feature attribution revealed by \methodname{}.  
For each class, we show generated images that activate the target neuron, the corresponding GradCAM visualizations, and the highest-scoring lexical units in $D_{\text{best}}$. These examples illustrate how non-causal cues (e.g., contextual elements, co-occurring objects, or geometric patterns) can dominate the classifier’s decision process.}
\label{fig:spurious_discovery}
\end{figure*}


A central objective of model dissection is not only to recover the intended semantic concept associated with a class, but also to expose the unintended cues a classifier relies on when making its predictions. Deep models frequently learn to associate target labels with non-causal regularities in the training data, such as backgrounds, co-occurring objects, or simple geometric patterns. Identifying these spurious cues is especially important in a strict black-box setting, where the auditor has no access to training data or internal activations.

\methodname{} naturally reveals such behavior as a byproduct of its optimization process. Because the prompt is refined solely through feedback derived from output probabilities, the procedure gravitates toward whatever visual patterns most strongly activate the classifier. By inspecting the high-confidence generated images, their corresponding GradCAM maps, and the lexical descriptors accumulated in $D_{\text{best}}$, we obtain a direct view of the non-causal features that the model treats as discriminative. Representative examples are shown in Fig.~\ref{fig:spurious_discovery}.

For ResNet50, the \textit{snorkel} class is often triggered by the presence of water, waves, or marine animals rather than by the snorkel apparatus itself. The \textit{baseball player} class displays a similar pattern: environmental cues associated with outdoor sports dominate over features specific to baseball, leading to confusion with classes such as soccer. A related issue arises in fine-grained categories such as \textit{daisy}, where the classifier focuses on background vegetation rather than flower morphology.

For ViT models, the reliance on scene-level or geometric regularities is even more pronounced. The \textit{space bar} class is activated by generic typing scenarios regardless of whether the actual key is visible. The \textit{horizontal bar} class frequently responds to straight-line structures; GradCAM often highlights the edge of an unrelated object whose geometry resembles the target class. Likewise, \textit{library} often activates in indoor educational environments such as classrooms or notice boards rather than canonical library scenes.

These qualitative findings provide important context for the quantitative results in Sections~\ref{sec:semantic_fidelity} and~\ref{sec:latent}. Since the purpose of \methodname{} is to reveal the classifier's actual reasoning process, any dependence on spurious cues should be reflected in the extracted descriptors. When this occurs, the recovered descriptors may diverge from the human-defined class semantics, and such divergence is expected. Lower similarity scores in some tables may therefore indicate genuine model bias rather than a shortcoming of the method. If the classifier strongly associates ``typing at a keyboard'' with the \textit{space bar} class, a descriptor aligned with this association accurately reflects its decision process, even if it deviates from the intended concept.


==> UNBOX/tex/experiments/zero_shot.tex <==
\label{zero_shot}

\subsection{Descriptors Evaluation}

We introduce a descriptor similarity evaluation protocol to quantitatively assess the quality of the textual descriptors generated by \methodname{}. Specifically, using the zero-shot classification capabilities of CLIP and Sentence Transformers we compute the accuracy score based on the semantic similarity between the features of the generated descriptors and different forms of ground-truth (e.g. class labels and data-driven descriptors).

Concretely, we compute similarity scores between descriptor and ground-truth allowing for standardized comparison across multiple semantic embedding spaces. Higher accuracy scores indicate stronger alignment with the underlying class semantics and, by extension, higher descriptor fidelity. Furthermore, we evaluate the visual grounding of the descriptors by treating them as pseudo-labels and measuring their correlation with corresponding validation images, thereby assessing their consistency with concrete visual evidence.



\input{tables/labels_zero_shot}
\subsubsection{Class labels}
\label{labels_zero_shot}
A primary objective of text-based explanation methods is to recover descriptors that faithfully characterize a target class and its consistently co-occurring attributes. To evaluate this property, we measure the semantic coherence of \methodname{}’s descriptors by directly comparing them against the ground-truth class labels. We operate under the assumption that an effective method should generate descriptors that exhibit significantly higher semantic similarity to the correct class label than to unrelated or semantically distant concepts.

We concatenate the top-5 class-level descriptors produced by \methodname{} into a single prompt and encode this prompt, together with the corresponding ground-truth label, using T5-XL. We compare our approach against three primary baselines: WWW and CLIPDissect, two state-of-the-art white-box methods that require access to full model weights and a probing dataset; and DEXTER, a grey-box method based on class activation maximization that relies solely on model weights. As a control, we additionally report results obtained using a pool of randomly sampled words.

The results, summarized in Tab.~\ref{tab:labels_zero_shot}, highlight the robustness of our approach across diverse architectures.
On RobustResNet50, \methodname{} achieves an accuracy of 0.70, significantly outperforming both WWW and DEXTER, and remaining highly competitive with CLIPDissect despite lacking access to model internals and data.

The strength of our optimization becomes even more evident when analyzing the other architectures. On ResNet50, \methodname{} reaches 0.77, matching the performance of CLIPDissect and surpassing WWW. Most notably, on ViT, \methodname{} achieves the highest accuracy, drastically outperforming CLIPDissect and WWW. This suggests that while white-box methods relying on internal activations may struggle to generalize across radically different architectures (e.g., CNNs vs. Transformers), \methodname{}'s output-driven approach maintains consistent interpretability capabilities regardless of the underlying model structure.


\input{tables/descriptors_zero_shot}
\subsubsection{Data-derived descriptors}
\label{data_der_zero_shot}
While the descriptor-label evaluation (\ref{labels_zero_shot}) confirms semantic coherence with the class subject, it is insufficient on its own. Comparing descriptors against a single textual label cannot reveal whether the method has identified important, co-occurring features or, conversely, known spurious features. More importantly, it cannot validate whether these discovered features are genuinely grounded in the data or are merely plausible-sounding artifacts generated by the explanation method.

To address this, we introduce a data-derived descriptor classification. We first constructed a set of data-grounded descriptors. To do this, we sampled 100 training images for each investigated ImageNet-1K class, captioned these images using LLaVA, and then extracted the top-5 most frequent keywords after excluding stop-words and noisy terms (e.g., \textit{"image," "picture"}). This process yields a set of descriptors representing concepts actually present in the data.

For evaluation, we concatenate the top-5 descriptors produced by \methodname{} and the data-derived descriptors into single prompts, which are then encoded using T5-XL. We compare the results of \methodname{} against those obtained by DEXTER, CLIPDissect, and WWW, as well as a random-word baseline serving as a control.

As shown in Tab.~\ref{tab:data_der_zero_shot}, CLIPDissect generally achieves high accuracy, benefiting from its full access to model weights and data. However, \methodname{} demonstrates consistent robustness and efficacy. On RobustResNet50, it achieves an accuracy of 0.60, outperforming WWW and performing comparably to DEXTER.

The advantage of our approach becomes clearer on standard architectures. On ResNet50, \methodname{} significantly surpasses WWW and narrows the gap with CLIPDissect. Most notably, on ViT, \methodname{} achieves the highest accuracy, substantially outperforming both CLIPDissect and WWW. This confirms that \methodname{}'s gradient-free optimization is particularly effective at extracting data-grounded features across diverse architectures, exhibiting superior generalization capabilities compared to methods relying on internal activation probing.

\input{tables/image_zero_shot}
\subsubsection{Visual Classification}
\label{image_zero_shot}
Finally, we evaluate the visual grounding of our class-level descriptors by performing a classification task directly on the ImageNet-1k validation set. While prior experiments demonstrated semantic coherence (\ref{labels_zero_shot}) and alignment with data-derived concepts (\ref{data_der_zero_shot}), this evaluation assesses whether the descriptors generated by \methodname{} correspond to features that are explicitly present in the visual data. For completeness, we include the ground-truth class labels as a practical upper bound and the data-derived descriptors as a data-grounded baseline.

We emphasize an important distinction in the experimental setup: for methods such as CLIPDissect and WWW, the validation set is also used as the probing set for concept extraction. In contrast, \methodname{} does not rely on validation data for descriptor discovery, ensuring a more stringent and unbiased evaluation of visual grounding.
As shown in Tab.~\ref{tab:image_zero_shot}, \methodname{} demonstrates remarkable performance. On RobustResNet50, \methodname{} achieves an accuracy of 0.58 surpassing WWW. On ResNet50, \methodname{} reaches 0.63 closing the gap with the data-derived ground truth.
Finally, on ViT, while lower than WWW, \methodname{} drastically outperforms CLIPDissect. 

These results provide strong evidence that \methodname{} is capable of extracting features that are genuinely grounded in the data distribution and have a tangible impact on the visual classifier's behavior, all while operating under the strictest black-box constraints.

==> UNBOX/tex/introduction.tex <==
\label{introduction}
\textit{Can the reasoning of a visual classifier be uncovered when the model is treated as a complete black box, with no access to its architecture, class definitions, training data, or learned weights?} Deep learning models have become the \textit{de facto} standard in computer vision, achieving state-of-the-art performance on a wide array of tasks. However, their remarkable empirical success is often offset by their inherent opacity. The high-dimensional, non-linear transformations learned within these models make their internal decision-making processes profoundly difficult for humans to interpret.

This challenge is significantly exacerbated in practice, as many of the most powerful and widely-adopted models are proprietary. They are often accessible only as inference APIs, with no public information on their training data, model weights, or even their architecture. This severe lack of access poses significant limitations, hindering our ability to debug failures, verify model reasoning, audit for fairness, or guarantee robustness. Consequently, adopting these models in high-stakes, safety-critical applications remains a persistent challenge, fueling a critical need for methods that can elucidate their internal workings under the strictest black-box constraints.

To address this critical lack of transparency, a significant body of research has focused on developing explainability methods, broadly categorized by their scope. \textbf{Local explanations} aim to interpret individual predictions by identifying which input features are most salient for a specific model's decision. \textbf{Global explanations} attempt to characterize the model's overall behavior. Finally, \textbf{slice discovery} aims to find subpopulations of a dataset (slices) that introduce systematic biases during model training. In recent years, the widespread adoption of Large Language Models (LLMs) has enabled a new class of text-based explanations across all three scopes. 

For local explanations, the Natural Language Explanations (NLE) field has received significant attention; works such as \cite{park2018multimodal, sammani2023uni, sammani2022nlx, hendricks2018grounding, zellers2018recognition} can explain per-sample model decisions with text by leveraging tasks like VQA. For global explanations, models like DiffExplainer \cite{DBLP:journals/corr/abs-2404-02618}, DEXTER \cite{carnemolla2025dexter}, and CLIPDissect \cite{oikarinen2023clipdissect} leverage LLMs, diffusion models, and VLMs to provide class-wise or neuron-wise model explanations or detect spurious features. DEXTER, for example, optimizes textual descriptors and outputs an LLM-generated bias report \cite{carnemolla2025dexter}, while CLIPDissect uses a concept vocabulary and a probing dataset to assign a descriptor to each neuron \cite{oikarinen2023clipdissect}. For slice discovery, powerful methods like B2T (Bias to Text) \cite{kim2024discovering} and LADDER \cite{ghosh2024ladder} use training data to retrieve textual keywords that describe biased slices, which can then be used for mitigation. However, these existing methods are fundamentally incompatible with the complete black-box scenario. Global techniques like DEXTER and CLIPDissect are, by design, white-box or grey-box; they require to know model weights. Similarly, leading slice discovery methods like B2T and LADDER require access to the original training data. This leaves a critical gap: \textit{understanding a model's reasoning when we are in a black-box and open-world scenario.}

A promising recent line of work introduced TextGrad \cite{yuksekgonul2024textgrad}, a general optimization framework that treats natural language feedback from LLMs as "textual gradients” to refine non-differentiable systems.

In this work, we propose \textbf{\methodname{}}, a novel, class-wise explanation framework that is entirely \textit{data-free and gradient-free}. \methodname{} is designed to describe a model's comprehension by discovering textual descriptors that strongly activate a specific class. Drawing inspiration from Dexter, \methodname{} combines a TextGrad-like optimization objective and Diffusion Models operating only on the model's output probabilities. We demonstrate on a subset of ImageNet-1K, Waterbirds, and CelebA that \methodname{} can successfully define and describe the class concepts encoded by a model without any prior knowledge of its architecture, weights, training data, or class definitions. We validate our framework through a series of rigorous evaluations: \textbf{(i) Ground-Truth Faithfulness:} A zero-shot classification task between our retrieved descriptors and ImageNet-1K class labels, demonstrating that our descriptors are semantically related to the class concept. \textbf{(ii) Semantic Coherence:} A zero-shot classification task comparing our descriptors to those extracted from the ImageNet-1K training images, proving their strong similarity. \textbf{(iii) Visual-Feature Correlation:} A zero-shot classification task against the ImageNet-1K validation set, showing our descriptors are strongly related to the visual features the class represents. \textbf{(iv) Slice discovery and debiasing:} on the Waterbirds and CelebA benchmarks, where our descriptors achieve results comparable to state-of-the-art methods that require access to training data or model weights. \textbf{(v) Human Evaluation:} we conduct a user study to perform human-based validation of relevance and accuracy with respect to the ImageNet-1K training images.

\vspace{5pt}
\noindent Our contributions are:
\begin{itemize}
    \item \textbf{A Novel Data and Gradient-Free Framework:} \methodname{} operates without access to model weights, gradients, architecture, or training data, using only the model's output probabilities. We introduce a novel optimization strategy that synergistically combines an agentic optimization and Diffusion Models.This approach reformulates activation maximization as a gradient-free search procedure, facilitating the discovery of textual descriptors that strongly activate a target class and naturally enabling a range of downstream applications, including model understanding, explainability, and semantic slice discovery.
    \item \textbf{Extensive Empirical Evaluation:} We demonstrate the effectiveness and broad applicability of our framework through comprehensive quantitative metrics and human-based evaluations on open-world and slice discovery benchmarks, including ImageNet-1K, Waterbirds, and CelebA. Our results show that the proposed method successfully defines and describes a model’s internal class concepts, producing descriptors that are semantically coherent, faithful to ground-truth concepts, visually relevant, and effective for downstream bias mitigation tasks.

\end{itemize}





==> UNBOX/tex/introduction_new.tex <==
\label{introduction}
\textit{Can the reasoning of a visual classifier be uncovered when the model is treated as a complete black box, with no access to its architecture, class definitions, training data, or learned weights?} As visual recognition increasingly relies on large proprietary models offered exclusively as inference APIs, this question has become central to trustworthy AI. In such deployments, users only observe output probabilities while all internal computations remain hidden, making it extremely difficult to understand why a classifier behaves the way it does, to diagnose failures, or to assess robustness and fairness in open-world settings.

A substantial body of work has explored the dissection of visual recognition models, aiming to uncover the internal concepts and mechanisms that drive their predictions. Local explanation methods, particularly Natural Language Explanations (NLEs) \cite{park2018multimodal, sammani2023uni, sammani2022nlx, hendricks2018grounding, zellers2018recognition}, focus on per-sample reasoning and often rely on multimodal supervision or VQA-style pipelines. In contrast, global explanation and model-dissection approaches aim to characterize a model’s overall conceptual space or the semantic attributes encoded in its representations. Recent methods such as DiffExplainer \cite{PENNISI2025104559}, DEXTER \cite{carnemolla2025dexter}, and CLIPDissect \cite{oikarinen2023clipdissect} use LLMs, diffusion models, or vision-language embeddings to optimize class-level descriptors, expose spurious features, or assign semantic labels to internal units and neurons. While these approaches provide valuable insight, they rely on access to model internals (weights, gradients, activations) or probing datasets. Other explanation strategies assume knowledge of the training distribution or annotated data. Consequently, none of these techniques can be applied in a black box scenario, where a model is only available through an API with no visibility into its architecture, parameters, or training data.

This gap emphasizes the need for a method that can perform global, class-wise model dissection using only a model’s output probabilities. Meeting this requirement demands a conceptual shift: rather than optimizing in feature space through gradients, which is impossible in black-box settings, we propose explanation as a semantic search problem driven entirely by natural language. Recent advances in textual optimization, such as TextGrad \cite{yuksekgonul2024textgrad}, show that LLM-mediated feedback can approximate gradient signals in non-differentiable systems, suggesting a promising direction for black-box interpretability. Motivated by this insight, we reformulate activation maximization as a gradient-free optimization loop carried out purely in text space. 
Building on this idea, we introduce \methodname{}, a class-wise explanation framework that is entirely \emph{data-free, gradient-free, and backpropagation-free}. \methodname{} discovers human-interpretable textual descriptors that strongly activate a target class using only the classifier’s output probabilities. The method combines a text-to-image diffusion model with an agentic, LLM-driven optimization mechanism that iteratively refines a natural-language descriptor for the target output neuron. A semantic guidance signal directs two cooperating LLM agents: one produces structured feedback and the other updates the descriptor. To ensure stability and prevent collapse onto narrow or transient descriptors, \methodname{} maintains a lightweight global and local optimization context that accumulates consistently high-reward prompts and salient lexical units while also tracking recent refinement steps. Through this combination, activation maximization is reformulated as a semantic optimization problem, enabling global model dissection without access to model architecture, parameters, or training data.
    
We evaluate \methodname{} on ImageNet-1K \cite{deng2009imagenet}, Waterbirds \cite{sagawadistributionally}, and CelebA \cite{liu2015deeplearningfaceattributes} through a comprehensive set of complementary tasks designed to assess fidelity, grounding, and practical utility. To measure semantic faithfulness, we compare our recovered descriptors against ground-truth class names and against descriptors extracted from training images via automated captioning.
To assess practical auditing capability, we use the descriptors to perform slice-discovery analysis on Waterbirds and CelebA, revealing spurious correlations and enabling debiasing despite having no access to training data or model internals. Across all tasks, \methodname{} achieves performance competitive with, and in several cases approaching, methods that rely on weights, gradients, or full training datasets, demonstrating its effectiveness as a fully black-box model-dissection tool.

\vspace{4pt}
To summarize, our main contributions are:
\begin{itemize}
\item A fully data-free and gradient-free framework for global model dissection. \methodname{} reconstructs class-level semantic concepts using only output probabilities, reformulating activation maximization as a text-space semantic optimization problem guided by diffusion-based evidence and agentic LLM reasoning.
\item A principled textual optimization mechanism that enables iterative refinement of descriptors through structured natural-language feedback without access to model weights, gradients, or training data.
\item Extensive evaluation across semantic, visual, and fairness-oriented tasks, showing that \methodname{} produces descriptors that are coherent, visually grounded, and effective for downstream auditing, including slice discovery and debiasing, despite operating in the strictest black-box setting.
\item Human validation of interpretability, demonstrating that the recovered descriptors are accurate, meaningful, and competitive with those produced by leading white-box explainability methods.
\end{itemize}


==> UNBOX/tex/limitations.tex <==
Despite its strong empirical performance, \methodname{} exhibits several limitations inherent to semantic optimization in discrete text space.\\

\noindent \textbf{Sensitivity to low-level or non-semantic visual cues}.
Because the optimization operates over natural-language descriptors, it inherently favors high-level, nameable concepts. When a classifier's decision depends mainly on low-level features—textures, fine-grained color patterns, or local shape primitives—the probability signal $s_t$ often responds only weakly to textual refinements.
A representative failure case is howler monkey: in ImageNet, many images contain dense foliage backgrounds with subtle texture–shape configurations. These cues are difficult to express linguistically, so the optimization receives a weak or noisy trend signal, leading to oscillations and poor convergence. In such settings, the method may fail to recover the true visual evidence used by the classifier.\\

\noindent \textbf{Computational cost of iterative refinement.}
Each optimization step involves two LLM forward passes and one diffusion-model rendering. On a system equipped with two H100 GPUs, a single step takes approximately 15 seconds, implying that full dissection of a class requires non-trivial compute. Although runtime scales with available hardware, this cost remains higher than that of single-pass attribution or gradient-based probing.

These limitations arise from the discrete linguistic search space and the reliance on large generative models for probing. Nonetheless, for the majority of classes, \methodname{} successfully uncovers stable, human-interpretable descriptors under strict black-box constraints.

==> UNBOX/tex/method/memory_bank.tex <==
\subsection{}

\label{memory_bank}
We observed that relying solely on the instantaneous signal from the $\mathcal{L}_t$ module (\ref{textual_loss}) was insufficient for navigating such a complex search space. The optimization could easily stagnate in local minima or discard successful concepts discovered in earlier iterations. By maintaining both long-term and short-term memory, we provide a feedback signal that captures the current optimization dynamics while preserving a global view of the overall process.


\subsubsection{Long-term Memory}
The long-term memory captures and accumulate the best prompts and the best semantic descriptors in order to persist known high-reward states that would be otherwise discarded. This memory is fed back into the Textual Optimization module (\ref{textual_optimization}) to augment the textual loss signal, preventing divergence and steering the search toward refining concepts already proven to be effective.

The \emph{best prompt extraction} process is implemented as an online filtering mechanism that is applied at each optimization step $t$.
A best prompt is defined as a complete textual prompt $p_t$ that, when passed through the Vision Pipeline (\ref{visual_pipeline}), generates an image $x_t$ resulting in a target class probability $s_t^{(j)}$ that exceeds a high-confidence threshold, $\tau_{best}$. If the probability $s_t^{(j)} \ge \tau_{best}$, the corresponding prompt $p_t$ and its score $s_t^{(j)}$ are stored in a candidate list $P_{best}$. At the conclusion of the entire optimization for a given class, this list $P_{best}$ is sorted in descending order by the probability score, providing a ranked list of the most effective full prompts discovered by the framework.

\emph{Semantic descriptors} are atomic, human-interpretable concepts (e.g., individual words) that serve as the fundamental building blocks of the generated prompts. The extraction of these descriptors is triggered whenever a prompt $p_t$ is added to the set $P_{best}$. Specifically, the selected prompt $p_t$ is parsed into its constituent tokens $\{w_i\} \in p_t$. After removing common stop-words, each remaining word $w_i$ undergoes an independent evaluation. We treat $w_i$ as a standalone prompt to synthesize a corresponding image $x_{w_i} = G(w_i, z)$ and subsequently query the classifier $\phi$ to obtain its individual probability score for the target class $j$:

\begin{equation}
	s_{w_i} = \phi(x_{w_i}, j).
\end{equation}
The resulting score $s_{w_i}$ quantifies the direct, individual contribution of each word to the activation of class $j$. Each word $w_i$, together with its corresponding score $s_{w_i}$, is stored in the candidate set $D_{best}$. Upon completion of the optimization process, $D_{best}$ is sorted in descending order according to $s_{w_i}$, yielding a ranked list of atomic semantic features that are most informative of the classifier’s internal representation of the target class.


At the conclusion of the optimization process, \methodname{} returns a pool of the best-performing prompts and semantic descriptors, ranked according to their activation scores. This accumulation mechanism enables a more holistic and generalized explanation of the target class. A classifier’s representation of a single class is often inherently multifaceted; for instance, the ``\textit{dogsled}'' class may be activated by diverse visual concepts such as ``\textit{snowy background}'', ``\textit{huskies}'', or ``\textit{humans in the snow}''. In contrast, a method that retains only the single best prompt from the final iteration would fail to reflect this rich, composite structure. By aggregating high-performing prompts and descriptors throughout the entire optimization trajectory, \methodname{} constructs a comprehensive set of semantic cues, yielding a more faithful and general representation of the class that captures the full spectrum of visual evidence on which the model relies.



\subsubsection{Short-term Memory}

The short-term memory component provides the Textual Optimization module with immediate temporal context by maintaining a sliding window over the most recent interaction steps. At each iteration $t$, the agent is supplied not only with the current optimization state, but also with a limited history of recent prompt-feedback pairs. This transient memory enables the system to remain aware of its recent decisions and their outcomes, allowing it to reason over local optimization dynamics.

Concretely, this mechanism serves two complementary roles. First, it mitigates redundant exploration by discouraging the reintroduction of prompts that have recently been identified as ineffective or erroneous. Second, it facilitates trajectory-aware refinement by allowing the agent to recognize and reinforce semantic changes that have empirically led to improvements in the target class activation. As such, short-term memory promotes stability and directional consistency in the iterative prompt refinement process.


\subsubsection{Unified Objective}
When jointly considering both long-term and short-term memory, the optimization process is guided by a holistic view that balances global semantic knowledge with local optimization dynamics. Long-term memory preserves a cumulative record of the best-performing prompts and descriptors, fostering global coherence and semantic diversity, while short-term memory captures the immediate trajectory of recent updates, preventing oscillations and unproductive cycles.

Formally, the prompt update rule defined in Eq.~\ref{eq:text_optim_pipeline} can be reformulated as:
\begin{equation}
p_{t+1} = A_u\!\big(p_t,\; A_f(p_t, \mathcal{L}_t, C_t, P_{best}, D_{best})\big),
\end{equation}
where $C_t$ denotes the short-term context window, and $(P_{best}, D_{best})$ represent the long-term memory of high-performing prompts and semantic descriptors. This unified formulation enables temporally-aware and semantically-informed optimization, yielding more stable, faithful, and generalizable class descriptions over the course of the iterative process.







==> UNBOX/tex/method/method_core.tex <==
\label{sec:method}

\begin{algorithm}[t]
\caption{Semantic optimization procedure used by \methodname{} to recover class-level descriptors from a black-box classifier.}
\label{alg:unbox}
\begin{algorithmic}[1]

\Require Classifier $\phi$, generator $G$, target class $j$
\Require Agents $A_f$ (Feedback), $A_u$ (Updater)
\Require Global Context $P_{\text{best}}, D_{\text{best}} \gets \emptyset$
\State Initialize prompt $p_0$

\For{$t = 0$ to $T$}
    \State Generate image $x_t \gets G(p_t)$
    \State Score $s_t \gets \phi(x_t)_j$
    \State Compute trend $T_t$ and intensity $I_t$
    \State Build semantic signal $S_t$
    \If{$s_t \ge \tau_{\text{best}}$}
        \State Add $(p_t, s_t)$ to $P_{\text{best}}$
        \State Extract lexical units and update $D_{\text{best}}$
    \EndIf
    \State $e_t \gets A_f(p_t, S_t, P_{\text{best}}, D_{\text{best}})$
    \State $p_{t+1} \gets A_u(p_t, e_t)$

\EndFor

\State Sort $D_{\text{best}}$ by activation score
\State \Return top-$k$ descriptors from $D_{\text{best}}$
\end{algorithmic}
\end{algorithm}


\methodname{} performs class-wise model dissection by iteratively refining a textual description so that, when rendered by a generative model, it maximally activates a chosen output neuron on a target classifier. The entire optimization takes place in \emph{semantic space}, i.e., the space of natural-language descriptors, because the classifier exposes neither gradients, architecture, nor training data. Formally, let 
\[
\phi : \mathcal{X} \to [0,1]^C
\]
be the classifier treated as a black box, and let $j \in \{1,\dots,C\}$ denote the target class. At iteration $t$, the method maintains a textual descriptor $p_t$, which is converted into an image through a pretrained text-to-image diffusion model $G$:
\[
x_t = G(p_t).
\]
The synthetic image is then evaluated by the classifier, which returns the
activation of the target output unit:
\[
s_t = \phi(x_t)_j.
\]
This scalar represents the model’s confidence that the generated sample
belongs to class $j$, and is the \emph{only} numerical feedback
available. 
The challenge is therefore to transform this single
probability value into an
optimization signal that can guide how the textual descriptor $p_t$ should be
updated. \methodname{} addresses this by interpreting the temporal evolution
of $s_t$ through two continuous quantities, \emph{trend} and
\emph{intensity}, which summarize the direction and magnitude of
progress, respectively.


\emph{Trend} captures whether the descriptor is improving with respect to the target class. It compares the current score $s_t$ to an exponential moving average of past scores,
\[
\bar{s}_{t-1} = \alpha s_{t-1} + (1-\alpha)\bar{s}_{t-2},
\]
and defines the deviation
\[
T_t = s_t - \bar{s}_{t-1}.
\]
Positive values indicate upward progress, negative values indicate deterioration, and near-zero values indicate stagnation. We discretize this continuous quantity into a semantic category:
\[
\text{trend\_state}(T_t) =
\begin{cases}
\texttt{up}, & T_t > \varepsilon,\\[4pt]
\texttt{down}, & T_t < -\varepsilon,\\[4pt]
\texttt{flat}, & |T_t| \le \varepsilon,
\end{cases}
\]
with a tolerance $\varepsilon > 0$. 
This categorical state acts as a symbolic cue for the language model, indicating the direction in which the descriptor should evolve.

\emph{Intensity} measures how far the descriptor is from producing a high activation and determines how strong the next update should be. It is defined as a margin-based proximity function:
\[
I_t = \max\{0,\ \tau_{\mathrm{high}} - s_t\},
\]
with $\tau_{\mathrm{high}}$ being a hyperparameter.
A large $I_t$ indicates the prompt is far from saturating the target unit, while small values indicate closeness to an optimal descriptor. As with trend, intensity is discretized when communicating with the language model:
\[
\text{intensity\_state}(I_t) \in \{\texttt{strong},\ \texttt{moderate},\ \texttt{micro}\},
\]
corresponding respectively to coarse, mid-scale, or fine-grained modifications to the current descriptor. These categories loosely resemble the effect of the learning rate in gradient-based methods, although all updates occur purely in linguistic form.

The discretized trend and intensity values
are used to 
index
two lookup tables containing short natural-language templates,

mapping each semantic state to a
corresponding textual instruction.

Selecting
the appropriate entries from these tables and concatenating them yields the
semantic guidance signal \(\mathcal{S}_t\) used by the LLM agents:
\[
\mathcal{S}_t
=
\mathbf{A}\big[\text{trend\_state}(T_t)\big]
\;\Vert\;
\mathbf{B}\big[\text{intensity\_state}(I_t)\big],
\]
where \(\mathbf{A}\) and \(\mathbf{B}\) denote the trend and intensity lookup
tables, respectively, and \(\Vert\) denotes string concatenation.


Once the semantic signal $\mathcal{S}_t$ is composed, it drives the update of the
descriptor through two cooperating LLM agents that operate in sequence. The
first is the \emph{Feedback Agent} $A_f$, which receives the current prompt
$p_t$ together with $\mathcal{S}_t$ and produces a structured natural-language
critique $e_t$ indicating how the descriptor should be modified to better
reflect the concept associated with the target output neuron $j$. The second is
the \emph{Updater Agent} $A_u$, which integrates this critique and returns a
refined prompt:
\[
p_{t+1} = A_u\big(p_t,\ e_t = A_f(p_t,\mathcal{S}_t)\big).
\]

Figure~\ref{fig:system_prompts} illustrates the system prompts that govern $A_f$
and $A_u$, together with the lookup table that converts the trend and intensity
states into the textual components of $\mathcal{S}_t$. The prompt of $A_f$
specifies its objective (maximizing the activation of class $j$), the inputs it
receives (current descriptor, semantic signal, and contextual cues from
high-scoring lexical units), and the strategy for producing concise and
actionable edits. The prompt of $A_u$ defines how these edits must be applied,
enforcing constraints on linguistic fluency, subject preservation, and prompt
length. The lookup table provides short, standardized fragments encoding the
direction and magnitude of semantic change, ensuring that $\mathcal{S}_t$ is
constructed through a controlled and reproducible mapping rather than an
unconstrained textual heuristic.

Depending on the direction and magnitude encoded in $\mathcal{S}_t$, the update
step may introduce new semantic attributes, suppress misleading or
non-discriminative elements, adjust the global scene configuration, or apply
fine-grained refinements to the existing description. In this way,
$\mathcal{S}_t$ modulates the scale and nature of the edit proposed by $A_f$ and
executed by $A_u$, ensuring that each iteration reflects a principled response
to the classifier’s feedback.


\begin{figure*}[h]
    \centering
    \includegraphics[width=1\textwidth]{figs/system_prompts.png}
    \caption{Excerpts of the system prompts for $A_f$ and $A_u$, along with the look-up table used to retrieve the text associated with $T_{s_t}$ and $I_{s_t}$ for the formulation of $\mathcal{S}_t$.}
    \label{fig:system_prompts}
\end{figure*}


==> UNBOX/tex/method/method_intro.tex <==
\label{method_intro}
\methodname{} performs class-wise model dissection by searching directly in
\emph{text space} for a natural-language prompt that maximally activates a
target output neuron of a black-box classifier. The method is organized into
two complementary components. First, the \emph{semantic optimization mechanism}
interprets the temporal evolution of the classifier’s output probabilities and
translates this signal into structured natural-language instructions that
iteratively refine the prompt. Second, the \emph{global and local optimization
context} stabilizes this refinement process by accumulating high-reward
semantic cues and by preserving short-range optimization history, thereby
providing both global coverage and local consistency. Together, these
components enable \methodname{} to recover a coherent and comprehensive textual
description of the concept encoded by the target class.
The overall pipeline of \methodname{} is shown in Alg.\ref{alg:unbox} and Fig.\ref{fig:method}.




==> UNBOX/tex/method/semantic_consolidation.tex <==
The optimization process described above operates entirely in semantic space and is therefore highly non-convex: many intermediate prompts may yield transient spikes in class activation without representing stable or meaningful aspects of the underlying concept. We noticed that relying solely on the semantic signal $\mathcal{S}_t$ leads to brittle behaviour: for instance, promising semantic attributes may be discarded and useful refinements overwritten. Most importantly, the absence of an explicit mechanism to leverage optimization history may cause the process to oscillate or stagnate.

To counteract these effects, \methodname{} maintains two complementary structures that summarize information across distinct temporal scales: (i) a \textit{Global Optimization Context}, which aggregates high-scoring prompts and their most relevant lexical units, and (ii) a \textit{Local Optimization Context}, which stores the most recent prompt--feedback interactions. These structures provide high-level semantic cues to the LLM agents without modifying the mathematical optimization signals (trend and intensity).\\ 

\noindent\textbf{Global Optimization Context.}
This component stores all prompts that achieve an activation above a high-confidence threshold $\tau_{\text{best}}$. Whenever $s_t \ge \tau_{\text{best}}$, the corresponding prompt $p_t$ is added to a set $P_{\text{best}}$. After optimization, this set is ranked by activation score, yielding a collection of the most effective prompts discovered for the target class.

To uncover finer-grained semantic cues, each selected prompt $p_t$ is decomposed into its lexical units $\{w_i\}$. After discarding items that do not constitute meaningful standalone semantic units (e.g., stop-words, conjunctions, determiners, auxiliary verbs), the remaining lexical items are treated as candidate semantic concepts. Each is independently evaluated by synthesizing an image from its single-word prompt:
\[
x_{w_i} = G(w_i), \qquad s_{w_i} = \phi(x_{w_i})_j.
\]
A concept set $D_{\text{best}}$, of maximum size $m$, stores the $w_i$ terms with the largest classifier activation $s_{w_i}^j$ obtained up to the current iteration, resulting
in a list of atomic semantic cues that strongly correlate with the targeted class.
These cues represent persistent high-reward concepts that should continue to influence future refinements even if they do not appear in the current descriptor.

This mechanism captures the multifaceted nature of class representations. For example, the class \emph{dog sled} may be activated by \textit{huskies}, \textit{snow}, \textit{sled}, or \textit{people in winter clothing}. A purely iterative update may converge to only one such attribute; the Global Optimization Context preserves the full semantic spectrum uncovered during exploration.\\

\noindent\textbf{Local Optimization Context.}
Alongside global structure, \methodname{} maintains a short sliding record of the most recent prompt-feedback interactions. This local context makes the optimization trajectory explicit: it prevents reintroducing recently rejected prompts and highlights refinements that have consistently improved the activation score over the last few steps.

Formally, the context $C_t$ stores a fixed-length sequence of recent pairs
\[
\{(p_{t-k},\, e_{t-k})\},
\]
where each $p_{t-k}$ is a past descriptor and each
\[
e_{t-k} = A_f(p_{t-k},\, \mathcal{S}_{t-k})
\]
is the critique generated by the Feedback Agent. By exposing $C_t$ to $A_f$, the system can amplify promising semantic directions, avoid short-term oscillations, and achieve smoother progression through the high-dimensional semantic search space.

Both the Global Optimization Context $(P_{\text{best}}, D_{\text{best}})$ and the Local Optimization Context $C_t$ are supplied to the LLM agents as auxiliary guidance. This yields a context-aware update rule of the form:
\[
p_{t+1} =
A_u\!\Big(
    p_t,\;
    A_f\big(p_t,\; \mathcal{S}_t,\; C_t,\; P_{\text{best}},\; D_{\text{best}}\big)
\Big).
\]

Iterations continue until the score evolution indicates convergence or a fixed iteration budget is reached. At that point, the set of best lexical units ($D_{best}$) is ranked by activation score, producing a collection of the most effective prompts discovered for the target class.



==> UNBOX/tex/method/textual_loss.tex <==
\label{textual_loss}
The \emph{Textual Loss} module serves as a state-tracking component that translates the numerical probability $s_t^{(j)}$ from the Vision Pipeline into a heuristic, natural-language prompt $\mathcal{L}_t$. This prompt serves as a ``loss signal'' that encapsulates the current system state and optimization progress, and is subsequently passed to the \emph{Textual Optimization} module to guide its next action. At the initial iteration ($t=0$), the module outputs a default initialization prompt $\mathcal{L}_{init}$ to cold-start the optimization process. For all subsequent iterations ($t > 0$), it computes two key metrics to characterize the system state: \textbf{Trend} ($T_s$) and \textbf{Intensity} ($I_s$).


\noindent\textbf{Trend.} This metric determines whether the system is improving, stagnating, or regressing. To mitigate high-frequency noise, we compare the current score $s_t^{(j)}$ against a dynamic baseline computed over a short-term sliding window. Let $H_s = \{s_{t-k}^{(j)}\}_{k=1}^{K}$ denote the history of the previous $K$ probability scores. We compute the window mean $\mu_s$ as the reference for trend estimation.


An \textbf{adaptive stability threshold}, denoted by $\epsilon_s$, is introduced to robustly identify a ``flat'' trend. The probability trend, $T_s$, is then determined by comparing $s_t^{(j)}$ to the baseline $\mu_s$:
\begin{equation}
    T_s =
    \begin{cases}
    \text{``up''} & \text{if } s_t^{(j)} > \mu_s + \epsilon_s \\
    \text{``down''} & \text{if } s_t^{(j)} < \mu_s - \epsilon_s \\
    \text{``flat''} & \text{otherwise}
    \end{cases}
    \label{eq:trend}
\end{equation}

\noindent\textbf{Intensity.} This metric captures the absolute magnitude of the current probability score $s_t^{(j)}$. We interpret it as the signal ``intensity'' and discretize it into three categorical states using two thresholds: a high-probability threshold $\tau_{\text{high}}$ and a low-probability threshold $\tau_{\text{low}}$. A ``micro'' intensity indicates that the current descriptors are already effective and require only minor refinements, whereas a ``strong'' intensity suggests that the descriptors are far from the target concept and require substantial modifications. The resulting intensity state $I_s$ is defined as:

\begin{equation}
    I_s =
    \begin{cases}
    \text{``micro''} & \text{if } s_t^{(j)} \ge \tau_{\text{high}} \\
    \text{``moderate''} & \text{if } \tau_{\text{low}} \le s_t^{(j)} < \tau_{\text{high}} \\
    \text{``strong''} & \text{if } s_t^{(j)} < \tau_{\text{low}}
    \end{cases}
    \label{eq:intensity}
\end{equation}

Finally, the textual loss prompt $\mathcal{L}_t$ is assembled from the combination of $T_s$ and $I_s$. A \textit{base} prompt is selected from a pre-defined dictionary based on the probability trend $T_s$, and a \textit{tail} prompt is appended based on the current Intensity $I_s$.




==> UNBOX/tex/method/textual_optimization.tex <==
\label{textual_optimization}
The Textual Optimization module is the core reasoning engine of the \methodname{} framework. It functions as a gradient-free optimizer that, inspired by TextGrad \cite{yuksekgonul2024textgrad}, replaces numerical gradients with structured, natural-language reasoning. Its objective is to take the heuristic ``loss signal'' $\mathcal{L}_t$~(\ref{textual_loss}) and generate a new, improved prompt $p_{t+1}$ for the next iteration.

This module is implemented using two distinct Large Language Model (LLM) agents operating in sequence: the Feedback Agent $A_f$ and the Updater Agent $A_u$.

The \emph{Feedback Agent} emulates a textual backward pass. At each step $t$, it receives as input the current prompt $p_t$ and the corresponding textual loss string $\mathcal{L}_t$. Based on this information, the agent $A_f$ analyzes the system state and generates a feedback signal $e_t$ in the form of a natural-language string that proposes modifications to $p_t$ with the objective of maximizing activation for the target class $j$. Early in the optimization, the feedback remains coarse and high-level, while progressively becoming more fine-grained as the process advances.

The \emph{Updater Agent} performs the actual optimization step. It takes as input the feedback signal $e_t$ together with the current prompt $p_t$, and is tasked with generating an updated prompt $p_{t+1}$ that explicitly incorporates the provided guidance. For instance, the agent may be instructed to refine $p_t$ by modifying specific attributes (e.g., altering the background), to merge $p_t$ with a descriptor drawn from $D_{best}$, or to discard $p_t$ entirely and propose a new variant.

Overall, the Textual Optimization module iteratively refines the prompt through a structured reasoning process that mimics backpropagation in the linguistic space, progressively steering the prompt toward higher activation and semantic alignment with the target class. This closed-loop update can be expressed as:
\begin{equation}
\label{eq:text_optim_pipeline}
p_{t+1} = A_u\!\big(p_t,\, A_f(p_t, \mathcal{L}_t)\big).
\end{equation}

where the Feedback Agent $A_f$ generates a natural-language correction signal based on the current prompt and loss, and the Updater Agent $A_u$ integrates this feedback to produce the next optimized prompt.







==> UNBOX/tex/method/vision_pipeline.tex <==
\label{visual_pipeline}
The \textbf{vision pipeline}, serves as the generative and evaluative component of our framework. Its objective is to compute a probability score $s_t^{(j)}$ that quantifies the effectiveness of a prompt $p_t$ in activating the target class $j$. This pipeline consists of a pre-trained text-to-image generator $G$ and the visual classifier $\phi$ under analysis.


At each iteration $t$, the generator $G$ takes the current textual prompt $p_t$ and a sampled noise vector $z \sim \mathcal{N}(0, \mathbf{I})$ as input to produce a synthetic image $x_t = G(p_t, z)$. The target classifier $\phi$ is treated as a complete black box. We assume an oracle-like setting in which, given an image $x$ and a target class index $j$, the model returns \textbf{only} the probability score $s^{(j)}$ associated with that specific class:

\begin{equation}
	s^{(j)}_t = \phi(x_t, j) \quad \text{where} \quad s^{(j)}_t \in [0, 1]
\end{equation}


==> UNBOX/tex/related.tex <==
\label{related_work}

\textbf{Visual classification explainability.} Modern visual classifiers often suffer from a lack of interpretability, which raises concerns regarding trust, reliability, and fairness in real-world applications. As a result, a substantial body of research has emerged to improve the explainability of these models, seeking to make their internal reasoning more transparent and human-understandable.

Existing approaches to explainability can be broadly categorized as \textit{intrinsic} or \textit{post-hoc} methods. Intrinsic approaches aim to design inherently interpretable models \cite{elton2020self, yang2023language}, while \textit{post-hoc} methods analyze pre-trained models to uncover the rationale behind their predictions.
Additionally, explanation methods can be \textit{local}, for interpreting single instances, or \textit{global}, providing insight into the model’s overall decision boundaries for all possible classes.

\noindent\textbf{Attribution-based methods.} Early approaches to \textit{post-hoc} visual model (VM) interpretability relied on \textbf{feature visualization} techniques, designed to expose the internal representations learned by neural networks, aiming to identify which pixels, segments or regions of an input image contribute most to a model’s decision, typically visualized through saliency maps or heatmaps \cite{simonyan2013deep, selvaraju2017grad, sundararajan2017axiomatic}. Although intuitive, early activation maximization (AM) approaches often produced unrealistic and uninterpretable visualizations. Subsequent work improved their generated image quality, with an example being DiffExplainer \cite{DBLP:journals/corr/abs-2404-02618}, which introduced soft prompts as diffusion-based generation strategy; nevertheless, these methods remain weakly interpretable and tend to yield fragmented feature mixtures \cite{nanfack2024adversarial, borowski2020exemplary}.

To overcome these limitations, a large portion of visual explainability research focuses on building more efficient and interpretable feature attribution methods \cite{selvaraju2017grad, sundararajan2017axiomatic, li2019beyond, wang2020score, han2023explainable}. Newer approaches can be grouped in two categories: 

\begin{itemize}
    \item Gradient-based methods backpropagate gradients to measure pixel influence \cite{selvaraju2017grad, zeiler2014visualizing, srinivas2019full};
    \item Perturbation- and counterfactual-based methods modify or remove image regions to observe the effect on model outputs \cite{fong2017interpretable, wagner2019interpretable, yu2022towards}.
\end{itemize}

These methods, which typically provide local insights, are usually sensitive to noise and can introduce subjective bias in interpretation \cite{kim2024discovering}. Moreover, by simply highlighting influential regions, they do not necessarily explain what aspect (e.g., color, shape, texture) drives the prediction, thus requiring human interpretation.


Frameworks for model-agnostic attribution, like LIME \cite{ribeiro2016should} and SHAP \cite{lundberg2017unified}, seek to mimic the behavior of black-box models on a local scale by employing interpretable surrogate models. Another approach involves the distillation of complex models into simpler alternatives \cite{jaakkola2018towards, chen2019looks}. Nonetheless, these methods inherently face information loss relative to the original model due to their reliance on simplified substitutes.



\noindent\textbf{Concept-based explanations.} Recent work attempts to explain model behavior and class separation thresholds through human-understandable concepts (e.g., shapes, colors, textures, actions appearing in images), also useful for debiasing and identifying spurious features. Concept-based VC explanation methods can refer to a single neuron, specific layers, or explain the model's predictive behavior as a whole \cite{bau2017network, oikarinen2023clipdissect, hernandez2021natural, wang2022hint, ahn2024unified}. Usually, they depend on annotated images or segments and require access to the internal states or representations of the model. A number of newer developments try to mitigate dependency from input data, nevertheless keeping their anchoring to model's weights. Instead, our proposed method – \methodname{} – is specifically designed for obtaining intuitive, textual global feedback on any visual classifier in a fully black-box (\textit{no data}, \textit{no weights}) setting.

\begin{itemize}
    \item The earliest approaches identify concepts with specific annotated images. The main ones are T-CAV \cite{kim2017interpretability}, T-CAR \cite{crabbe2022concept}, IBD \cite{zhou2018interpretable}, and, more recently, CRAFT \cite{fel2023craft}. T-CAV quantifies the contribution of a given concept, represented by guide images, to a target class in a specific layer of the model. To do this, it involves training a linear probe with sets of positive and negative images. The Concept Activation Vector (CAV) that separates the two sets is used to calculate the T-CAV score, which measures the sensitivity of the model to a given concept in predicting the respective class. T-CAR is the non-linear evolution of T-CAV, which identifies Concept Activation Regions (CAR) with a kernel-based SVM method, so as to identify each concept with a region in space rather than with a vector. IBD performs an optimization to assess the relevance of concepts with respect to classes. CRAFT, in turn, leverages non-negative matrix factorization to identify CAVs and localize the most relevant input regions for each CAV. However, these methods are not only data-dependent, but also do not immediately translate the results into human-understandable terms.
    
    \item More recent approaches adopt textual concepts and therefore provide more intuitive explanations. Some are bound to pre-defined textual concept sets (for instance, annotated datasets, human input, or \textit{top-k} words corpora). This category includes:
    
    \begin{itemize}
        \item Natural Language Explanations (NLE) \cite{park2018multimodal, hendricks2018grounding, sammani2022nlx, sammani2023uni, zellers2018recognition} aim to provide rationalizations of VC predictions explaining the evidence for a decision, e.g. by adopting VQA benchmarks \cite{park2018multimodal, sammani2022nlx, sammani2023uni, zellers2018recognition}, in contrast to methods that just show intermediate activations. 
        Pioneering work in NLE for vision-language tasks explored multimodal supervision and explanation grounding. Multimodal Explanations \cite{park2018multimodal} introduces an LSTM–CNN model trained on human-provided textual and visual justifications, leveraging attention mechanisms to localize salient image regions supporting the rationale, evaluated on both VQA and activity recognition benchmarks. 
        Grounding Visual Explanations \cite{hendricks2018grounding} further advanced this line by generating debiased, image-relevant explanations through contrastive training with negative phrases, producing both counterfactual statements and justifications for the predicted class. While early work relied on separate modules for feature extraction, prediction, and explanation \cite{park2018multimodal, hendricks2018grounding, zellers2018recognition}, Uni-NLX \cite{sammani2023uni}, extending \cite{sammani2022nlx}, unifies NLE tasks into a single causal language-modeling framework that treats explanations as text generation, enabling a compact multi-task model based on an LLM. 
        NLE-style methods, however, remain local and supervised.
        \item Bottleneck-based methods \cite{koh2020concept, yang2023language} perform global debiasing on VCs by building bottleneck layers and increasing the set of descriptive words for a class, e.g., by including a human in the loop \cite{koh2020concept} or by prompt-tuning an LLM \cite{yang2023language}.
        \item Global dissection methods operating at neuron and layer level, such as NetworkDissection \cite{bau2017network} and Net2Vec \cite{fong2018net2vec}, link human concepts to individual filters by computing the \textit{IoU} overlap between segmentation masks and feature maps, thereby identifying which concept each neuron most strongly represents. Concept Aware Explainability (CAE) \cite{gurkan2025concept} employs a densely annotated segmentation dataset to identify the best set of filters for each concept and the best set of concepts for each filter. HINT \cite{wang2022hint} and MILAN \cite{hernandez2021natural} train concept classifiers to reduce matched data annotation dependency. Other methods use CLIP's latent space to align images and text: CLIPDissect \cite{oikarinen2023clipdissect} labels internal neurons with open-ended concepts by introducing a concept-activation matrix constructed through the inner products of textual and visual embeddings to identify the most similar concept for each unit, allowing detached use of any VC with any corpus of textual concepts; CounTEX \cite{kim2023grounding} produces counterfactual explanations of images starting from CLIP-derived label embeddings; WWW \cite{ahn2024unified}, designed to be able to address the \textit{what}, \textit{where} and \textit{why}s of black-box VCs decisions in human understandable terms, starts from CLIP-extracted class concepts and generates class and sample concept maps and heatmaps by combining Shapley values with neuron activation maps (NAM).
    \end{itemize}

    \item Another branch of concept-based approaches has proven suitable for explaining visual models in scarce input data settings and work without annotated probes. Within those, textual concepts are generated through some kind of optimization process.
    Traditional, gradient-based optimization is employed in works such as TEXplain \cite{asgari2024texplain}, which subjects the visual features of the model to a Large Language Model (LLM) in order to find the concepts that describe its behavior; GIFT \cite{zablocki2024gift}, that generates textual explanations with an LLM starting from counterfactual signals; DEXTER \cite{carnemolla2025dexter}, which provides class-wise textual reports through a gradient-based textual optimization process, without the need for annotated data.

     \methodname{}, our proposed contribution, represents an innovation compared to all previous approaches, because it adopts a fully textual optimization pipeline, capable of explaining a totally black-box visual classifier while being unaware of its architecture, classes, weights and representations.
    \end{itemize}

\noindent\textbf{Slice discovery and debiasing.} Despite being able to achieve high average accuracy in classification tasks, deep neural networks often fail systematically on specific subsets of data, known as \textit{error slices} \cite{yu2022towards, ghosh2025ladder}. Slice discovery aims to identify these coherent subpopulations to reveal \textit{spurious}, i.e., non-causal correlations or distribution shifts that can hinder reliable generalization. Early approaches to slice discovery relied on predefined sensitive attribute banks (e.g., \textit{age}, \textit{gender}), which limited their ability to capture biases arising from data pre-processing or domain-specific factors \cite{ghosh2025ladder}.

Several recent frameworks address these limitations by inferring group labels automatically; however, their effectiveness depends heavily on the quality of the discovered groups. Bias-to-Text (B2T) \cite{kim2024discovering} discovers visual biases by extracting pseudo-labels from captions of misclassified images and validating them with a vision–language scoring model, enabling zero-shot bias labeling and debiased training without predefined bias sets. Similarly, LADDER \cite{ghosh2025ladder} leverages joint vision–language representations to detect slices where the classifier underperforms, but uses retrieved text and LLM-generated hypotheses to produce pseudo-labels for debiasing, requiring no paired annotations. 

In this context, we refer to Distributionally Robust Optimization (DRO) \cite{sagawadistributionally} as a core tool for debiasing, used to minimize the worst-case loss across groups and adopted by several slice discovery methods to compute accuracy on the identified slices. The original Group DRO (GDRO) formulation \cite{sagawadistributionally} shows that naïve DRO fails in overparameterized models due to perfect group-level fitting, and that strong regularization is essential for improving worst-group generalization. DRO typically requires explicit annotations for all samples; this requirement has been satisfied by some recent contributions with unsupervised inference of biased group labels. 

As notable examples, Learning from Failure (LfF) \cite{nam2020learning} is a slice discovery method that assumes and exploits the simplicity bias of neural networks by jointly training a biased and a debiased model, reweighting samples based on their loss trajectories to emphasize bias-conflicting examples without requiring spurious labels; GEORGE \cite{sohoni2020no} addresses hidden stratification by clustering features to estimate latent subclasses and then applying GDRO to improve worst-subclass accuracy. A similar but simpler and more effective approach is Just Train Twice (JTT) \cite{liu2021just}, employing two models to enhance worst-group performance: a standard Error Minimization Model (ERM) trained with regularization to identify misclassified samples; a second model, which upweights the examples from the poorly performing groups identified by the first model. This approach achieves better results than standard ERM and DRO, while only requiring a small set of annotated data for validation. Correct-N-Contrast (CNC) \cite{zhang2022correct} further upgrades this method without the need for attribute labels. Maintaining a two-model pipeline, CNC first identifies spurious correlations by training a ERM model with regularization, as done in JTT, but then uses these predictions for contrastive learning with a second model, where the sampling strategy chooses positive examples as samples from the same class but with different ERM predictions, and negative examples as samples from different classes but with the same ERM prediction, thus encouraging the replacement of learned spurious correlations in favor of genuinely causal class features. 

As shown in detail in Sect. \ref{slice_discovery}, we tested \methodname{} with slice discovery, comparing our results with all the previously referenced state-of-the-art methods \cite{yu2025error, ghosh2025ladder, kim2024discovering, sagawadistributionally, nam2020learning, sohoni2020no, liu2021just, zhang2022correct}.

\noindent\textbf{Text-based optimization for explainability.} A great deal of current research on explainability for deep learning models explores the use of generative Large Language Models as critics, optimizers, and self-assessing agents, enabling \textit{gradient-based} or \textit{gradient-free} refinement of models and explanations for various reasoning tasks, through In-Context Learning (ICL), training or architectural enhancements \cite{madaan2023self, press2023measuring, yao2023tree, weng2023large, hao2024training}. This trend aligns with cognitive frameworks, inspired by human brain functions, such as CoALA \cite{sumers2023cognitive}, that conceptualizes reasoning as reading and writing into a semantic memory through natural language, thus framing inference as a textual operation. This perspective has inspired the development of agentic approaches to self-supervised prompt optimization, like the TextGrad general framework \cite{yuksekgonul2024textgrad} for refining non-differentiable systems, and applications in tasks such as model inversion \cite{fei2023gradient} and adversarial attacks mitigation \cite{yuan2023bridge}.

However, the potential of textual gradients for explaining visual classifiers remains largely unexplored. \methodname{} extends this paradigm by employing LLM-driven textual optimization as a \textit{post-hoc}, model-agnostic and globally interpretable mechanism that integrates visual evidence, language grounding, and cognitive-style self-assessment, in a \textit{data-free} and \textit{gradient-free} setting.




==> UNBOX/tex/related_new.tex <==
A large body of work seeks to interpret visual classifiers by uncovering the internal concepts and mechanisms driving their predictions. Approaches differ along two axes: \textit{intrinsic} methods, which build interpretable models from the outset \cite{elton2020self, yang2023language}, and \textit{post-hoc} methods, which dissect pre-trained models to explain how they arrive at their decisions \cite{selvaraju2017grad, carnemolla2025dexter, oikarinen2023clipdissect, ahn2024unified}.
Both types of methods may provide \textit{local} explanations for individual samples or \textit{global} explanations describing the conceptual structure of the entire model. \methodname{} belongs to the latter category: a global post-hoc method for model dissection and explainability. In this section, we review prior work based on the assumptions they make about model and data access. We first review attribution-based approaches, which offer local insights but no global semantic structure. We then cover concept-based methods, that provide richer explanations but require internal weights, activations, or annotated concepts. Next, we examine global language-driven explanatory methods that perform textual optimization without explicit annotated probes. Finally, we discuss slice-discovery and debiasing frameworks that rely on access to the underlying data.

\noindent \textbf{Attribution-based local explainability.}
Early explainability work focused on attribution methods that highlight which regions of an input image influence a model’s prediction the most. These include feature visualization and saliency-map approaches \cite{simonyan2013deep, selvaraju2017grad, sundararajan2017axiomatic}, improved later by diffusion-based activation maximization techniques such as DiffExplainer \cite{PENNISI2025104559}. Other refinements expanded feature attribution to gradient-based methods \cite{selvaraju2017grad, zeiler2014visualizing, srinivas2019full} and perturbation-based methods \cite{fong2017interpretable, wagner2019interpretable}.

While these methods provide fine-grained insights, they are inherently \textit{local}, often noisy, and require human interpretation to infer the underlying semantic concepts \cite{kim2024discovering}. Model-agnostic surrogates such as LIME \cite{ribeiro2016should} and SHAP \cite{lundberg2017unified} attempt to explain predictions via simpler proxy models but inevitably suffer from information loss.
These methods cannot perform global model dissection and cannot operate in black-box settings, as they require model queries beyond class probabilities, gradients, or feature maps.

\noindent \textbf{Concept-based methods} aim to provide global explanations through human-interpretable semantic "concepts" (e.g., textures, colors, shapes, parts). Traditional approaches such as T-CAV \cite{kim2017interpretability}, T-CAR \cite{crabbe2022concept}, IBD \cite{zhou2018interpretable}, and CRAFT \cite{fel2023craft} require annotated examples or segmentation supervision to identify the relevance of concepts within internal layers.

More advanced variants perform neuron- or filter-level concept assignment. NetworkDissection \cite{bau2017network} and Net2Vec \cite{fong2018net2vec} link feature maps to interpretable units; CAE \cite{gurkan2025concept}, HINT \cite{wang2022hint}, and MILAN \cite{hernandez2021natural} improve concept localization and reduce annotation dependency. Other methods exploit CLIP embeddings: CLIPDissect \cite{oikarinen2023clipdissect} labels neurons with open-ended concepts, CounTEX \cite{kim2023grounding} generates counterfactual explanations, and WWW \cite{ahn2024unified} combines Shapley scores and neuron activation maps to answer the what/where/why of a decision.
Parallel to these, Natural Language Explanations (NLEs) \cite{park2018multimodal, hendricks2018grounding, sammani2022nlx, sammani2023uni, zellers2018recognition} generate textual rationales for predictions but are predominantly local, supervised, and task-dependent.

All these methods require access to model internals (weights, activations, layers, features) or annotated concepts. None can operate with only output probabilities, nor can they fully reconstruct class-level conceptual structures of a black-box model.\\

\noindent \textbf{Global language-driven model dissection}. Several recent methods have explored using textual optimization or generative models for concept-based explanations without explicit annotated probes. TEXplain \cite{asgari2024texplain}, GIFT \cite{zablocki2024gift}, and DEXTER \cite{carnemolla2025dexter} generate class-level descriptors through textual or multimodal optimization. However, these methods still depend on gradients, internal representations, or feature activations, and thus remain incompatible with strict black-box settings.

\methodname{} advances beyond these approaches by performing global, class-wise textual optimization without any access to data, weights, gradients, or internal activations.\\

\noindent \textbf{Slice discovery and debiasing.} Slice discovery seeks to identify coherent subsets of data where a model fails systematically, often as a result of spurious correlations or hidden stratification \cite{ghosh2025ladder}. Modern approaches such as B2T \cite{kim2024discovering} and LADDER \cite{ghosh2025ladder} rely on vision–language models or retrieved text to infer slices that lack explicit annotations. Distributionally Robust Optimization (DRO) \cite{sagawadistributionally} and its refinements \cite{nam2020learning, sohoni2020no, liu2021just, zhang2022correct} are then used to mitigate worst-group errors.

Although slice discovery and debiasing are not the primary objectives of \methodname{}, we show that the descriptors our method uncovers can be effectively used in slice-sensitive analysis and debiasing, performing competitively with approaches that require data access or model internals.
